Atomic Crosschain Transactions White Paper

Atomic Crosschain Transaction technology allows composable programming across private Ethereum blockchains. It allows for inter-contract and inter-blockchain function calls that are both synchronous and atomic: if one part fails, the whole call graph of function calls is rolled back. It is not based on existing techniques such as Hash Time Locked Contracts, relay chains, block header transfer, or trusted intermediaries. BLS Threshold Signatures are used to prove to validators on one blockchain that information came from another blockchain and that a majority of the validators of that blockchain agree on the information. Coordination Contracts are used to manage the state of a Crosschain Transaction and as a repository of Blockchain Public Keys. Dynamic code analysis and signed nested transactions are used together with live argument checking to ensure execution only occurs if the execution results in valid state changes. Contract Locking and Lockability enable atomic updates.

==> considerations.tex <==
\section{Other Considerations}

\subsection{Finality}
TODO: The definition of finality for parts of a crosschain call is blockchain dependent. For probabilistic finality blockchains, the definition of final needs to be agreed up by validators.

This assumption of having a threshold number of Byzantine validator nodes is the same type of assumption that Byzantine Fault Tolerant (BFT) consensus protocols make \cite{ibft, ibft2}.

\subsection{Threshold Settings}





==> limitation.tex <==
\section{Limitation}

The locking protocol induces a limitation. In our locking mechanism, after processing the function belonging to an originating or a subordinate transaction using given inputs, we lock the contract to which the function belongs to. Suppose one of the subordinate transactions makes a call to one of the functions in the locked contract (some function of which has already been processed in the current crosschain transaction), then that subordinate transaction fails, making the whole crosschain transaction to abort. Consider the function call-graph of a crosschain transaction. This function call-graph can be transformed to a {\em contract call graph} by replacing the functions with the contracts that they belong to. The locking mechanism limits a crosschain transaction not to have repeated contracts in its contract call graph. Note that by function call-graph and contract call-graph, we mean a dynamic function call-graph and a dynamic contract call-graph respectively, where infeasiblity (with respect to given inputs) of call-edges have been pruned out.

A partial solution is to restrict the granularity of locking to functions rather than contracts. It relaxes the above limitation to a degree where contracts can repeat in the contract call graph but functions cannot (disallows recursive functions). 

